Compute-Constrained Data Selection

Data selection can reduce the amount of training data needed to finetune LLMs; however, the efficacy of data selection scales directly with its compute. Motivated by the practical challenge of compute-constrained finetuning, we consider the setting in which both the cost of selecting data and training are budgeted for. We first formalize the problem of data selection with a cost-aware utility function, and model the data selection problem as trading off initial-selection cost for training gain. We run a comprehensive sweep of experiments across multiple tasks, varying compute budget by scaling finetuning tokens, model sizes, and data selection compute. Interestingly we find that many powerful data selection methods are almost never compute-optimal, and that cheaper data selection alternatives dominate both from a theoretical and empirical perspective. For compute-optimal training, we find that perplexity and gradient data selection require training-to-selection model size ratios of 5x and 10x, respectively.

==> sections/Theory/7_Theory.tex <==
\section{Theoretical Analysis of Compute Optimal Data Selection} 

\subsection{Modeling Expected Utility in Data Selection Under Computational Constraints}

We are interested in studying the trade-off between spending computational resources in either data selection or training and attempts to determine optimal strategy based on data concentration and method efficiency.

Given a dataset with size (\( D \)), a computational budget of  (\( K \)), and data selection method with cost $C_{DS}$, we can train a total of (\( M \)) data points where $ M = \frac{K - C_{\text{DS}}}{c_{\text{train}}}$.

Depending on what our target task is, the number of useful data within a given training dataset changes accordingly. Because of this, we introduce a bias term concentration (\( P \)) to denote the  fraction of data points that are high-utility (i.e. helpful to our target task). For convenience, we will assume each data point has a utility of 1 (high-utility) or 0 (null-utility). Following this, the number of high-utility data points is \( N = P \cdot D \).

\textbf{Expected Utility.} When data is selected randomly without any data selection effort (\( C_{\text{DS}} = 0 \)), the probability of selecting a high-utility data point is simply equal to the concentration: $
p_{\text{rand}} = P$. The expected utility under random selection is:
\[
U_{\text{rand}} = M_{\text{rand}} \cdot p_{\text{rand}} = \left( \frac{K}{c_{\text{train}}} \right) P.
\]

Spending computational resources in data selection (\( C_{\text{DS}} > 0 \)) essentially increases the probability of selecting high-utility data points but reduces the number of data points that can be trained on. To model the probability \( p(C_{\text{DS}}) \) as an increasing function of \( C_{\text{DS}} \), we formulate it as an exponential growth function:

\[
p(C_{\text{DS}}) = 1 - (1 - P) e^{- \beta C_{\text{DS}} }
\]

where \( \beta > 0 \) is a learned constant that determines the rate of increase, used to account for different data selection methods' varying efficiencies. Intuitively, $p(C_{\text{DS}})$ will be higher than $p_{\text{rand}}$ as we increase $C_{\text{DS}}$ ; meanwhile, the marginal value that one can get from increasing $p(C_{\text{DS}})$ should diminish.  The expected utility under data selection with $C_{\text{DS}}$ is:

\[
U_{\text{DS}}(C_{\text{DS}}) = M \cdot p(C_{\text{DS}}) = \left( \frac{K - C_{\text{DS}}}{c_{\text{train}}} \right) \left[ 1 - (1 - P) e^{- \beta C_{\text{DS}} } \right]
\]


The formulation in \Cref{Background 5} has a implicit goal of finding the optimal data selection cost \( C_{\text{DS}}^* \) that maximizes the expected utility \( U_{\text{DS}}(C_{\text{DS}}) \):

\[
C_{\text{DS}}^* = \underset{C_{\text{DS}}}{\arg\max}
\quad \text{subject to} \quad 0 \leq C_{\text{DS}} \leq K.
\]

Crucially, this formulation suggests that the optimal \( C_{\text{DS}}^* \) depends on the concentration \( P \): when \( P \) is small, high-utility data is rare. Spending more in data selection is beneficial to increase \( p(C_{\text{DS}}) \), so the optimal \( C_{\text{DS}}^* \) is higher. In contrast, when \( P \) is close to 1, high-utility data is abundant, and spending more directly in training helps more than selecting data.

\colorbox{yellow}{QUESTION: How do we map this to our results?} We use the current optimal results to fit the equation to obtain the constant $\beta$? I don't know how model size may effect the data selection. Larger model may utilize data differently despite having the same data, so $\beta$ might be method and model specific. Also are we assuming the utility here has a linear relation with our performance metric?



==> tables/Data_Select_Methods.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|}
\toprule
\textbf{Approach} & \textbf{Base} & \textbf{Word Frequency} & \textbf{N-Gram} & \textbf{Model Representation} & \textbf{Perplexity} & \textbf{Gradient Feature} \\ 
\midrule
\textbf{Method}  & Rand. & BM25 & DSIR & RDS  & Top-K & LESS   \\
\bottomrule
\end{tabular}}
\caption{Different Data Selection Approaches and Corresponding Methods.}
\label{tab:Data_Selection_Methods}
\end{table}


==> tables/Repeated_Data_Set_Up.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\textbf{FLOP budget $(C)$} & \textbf{Parameters $(N)$} & \textbf{Training tokens $(D)$} & \textbf{Epoch} & \textbf{Data budget $(D_C)$} \\ 
\midrule
$4.6 \times 10^{17}$ & \multirow{5}{*}{7B} & 5M  & \multirow{5}{*}{\{1,2,3,4,5\}}  & \{5, 2.5, 1.7, 1.3, 1\}M \\ 
$1.1 \times 10^{18}$ &  & 10M &   & \{10, 5, 3.3, 2.5, 2\}M \\ 
$2.3 \times 10^{18}$ &  & 25M &   & \{25, 12.5, 8.3, 6.7, 5\}M \\ 
$4.6 \times 10^{18}$ &  & 50M &   & \{50, 25, 16.7, 12.5, 10\}M \\ 
$9.2 \times 10^{18}$ &  & 100M&   & \{100, 50, 33.3, 25, 20\}M \\ 
\bottomrule
\end{tabular}}
\caption{Validation Loss for Different Data Constraints (IsoFLOP). Each curve represents the same number of FLOPs spent on an equal size model. Colors represent different numbers of epochs due to repeating because of data constraints. Parameters and training tokens are set to match the single-epoch compute-optimal configurations for the given FLOPs. Models trained on data that is repeated for multiple epochs have consistently worse loss and diverge if too many epochs are used.}
\label{tab:repeated_data_set_up}
\end{table}


==> tables/Target_task.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|}
\toprule
\textbf{Criteria} & \textbf{Factual Knowledge} & \textbf{Reasoning} & \textbf{Multilinguality} & \textbf{Coding} & \textbf{Safety}\\ 
\midrule
\textbf{Benchmark} & MMLU & BBH & TYDIQA & Codex-Eval & TruthFulQA   \\
\bottomrule
\end{tabular}}
\caption{Different Criteria of Evaluation and Corresponding Benchmarks.}
\label{tab:Target_task}
\end{table}


==> tables/Training_FLOPs.tex <==

\begin{table}[h]
\centering
\caption{Proposed training budgets based on the percentage of the total training tokens. For various model sizes, we show the estimations of FLOPs per token and the total FLOPs for training. (Details of calculation are shown in Appendix A.1).}
\label{tab:flops_tokens}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\textbf{Budget} & \textbf{Parameters} & \textbf{FLOPs per token} & \textbf{\% of Training Tokens} & \textbf{Tokens} & \textbf{FLOPs} \\
\midrule
Tiny & 70B & 4.36e+11 & 1 & 0.96 Million & 4.19e+17 \\ 
Small & 70B & 4.36e+11 & 5 & 4.79 Million & 2.09e+18 \\ 
Medium & 70B &4.36e+11 & 10 & 9.57 Million & 4.17e+18 \\ 
High & 70B &4.36e+11 & 20 & 19.14 Million & 8.35e+18 \\ 
\bottomrule
\end{tabular}
\label{tab:training_FLOPS}
}
\end{table}

